2FHL J0826.1-4500: Discovery of a possible shock-cloud interaction on the Western edge of the Vela SNR

We report on the investigation of a very high energy (VHE), Galactic gamma-ray source recently discovered at >50GeV using the Large Area Telescope (LAT) on board the Fermi-LAT. This object, 2FHL J0826.1-4500, displays one of the hardest >50GeV spectra (gamma-ray photon index ~1.6) in the 2FHL catalog, and a follow-up observation with XMM-Newton has uncovered diffuse, soft thermal emission at the position of the gamma-ray source. A detailed analysis of the available multi-wavelength data shows that this source is located on the Western edge of the Vela supernova remnant (SNR): the observations and the spectral energy distribution modelling support a scenario where this gamma-ray source is the byproduct of the interaction between the SNR shock and a neutral Hydrogen cloud. If confirmed, this shock-cloud interaction would make 2FHL J0826.1-4500 a promising candidate for efficient particle acceleration.

==> extra.tex <==
\section{Multi-wavelength Shock Presence and Implications}
\subsection{X-rays}
Vela is the closest SNR to Earth that houses a middle-aged pulsar (T$\approx$11kyr) with a distance of D$\approx$290pc \citep{grondin2013} making it a popular region to study. It is a fascinating research endeavor as the Vela region is complex in structure. The Vela pulsar sits in the central region of its supernova remnant (SNR) shell while actively fueling a pulsar wind nebula (PWN) $2\degree$x $3\degree$ in size known as Vela-X. Pulsar wind nebulae are magnetized winds of relativistic particles fueled by the pulsar's dissipated rotational energy and form at the wind termination shock (TS) that develops from the interaction of the surrounding SNR plasma and relativistic wind \citep{grondin2013}. Understanding the mechanisms in this region are critical to accurately interpreting the nature and evolution of PWNe, SNR and their hosts.

The structure of a composite SNR is complex and heavily depends on the density of the surrounding material it expands into. Figure 3 of \citet{pslane} includes a useful diagram on the layers of an SNR as it moves through the circumstellar medium (CSM) with a density gradient. The expansion of the PWN into the SNR and the SNR expansion into the CSM are both responsible for heating ejecta and ambient material. A high pressure bubble may form from the pulsar wind expanding into the SNR and as the bubbles expands supersonically through the ejecta, a shock front forms \citep{pslane}. The ejecta can confine the PWN and as the PWN expands into the ejecta it also drives a shock, heating the material and producing thermal emission. 

The Vela SNR is one of the brightest, largest soft X-ray sources. ROSAT has mapped the Vela region in the soft X-rays showing a large presence of diffuse X-ray emission that encompasses the Vela pulsar and roughly outlines the SNR shell that is 8$\degree$ in diameter. J0826-4500 lies along the edge of the PWN where the ROSAT X-ray emission drops off. A cavity is apparent in this region where little X-ray emission is present (Figure 4). \citet{bach2000} performed a spectral analysis on 3 distinct regions of the SNR to find that the X-ray emission is of thermal origin, best described by two-temperature Raymond-Smith thermal plasma models. This idea is consistent with what was have found with XMM-Newton.

\begin{figure}[!t]
\centering
\includegraphics[width=.75\linewidth]{ROSAT_cavity.png}
\caption{ROSAT image of western side of SNR. Green circle labels location of X-ray shock with a radius of 5'. Shock lies on edge of prominent X-ray shell just before a large cavity. The bright source in the top left corner is Puppis A.}\label{fig:rosat}
\end{figure}

{\color{red}Show overlay of ROSAT data with our shock. Discuss spectral analysis of ROSAT data and compare to our data. Is there a temperature gradient? Does our analysis fit with what F. J. Lu & B. Aschenbach found with the same ROSAT data?}

\subsection{Radio}
The Vela region is rich with radio emission, largely coming from Vela-X with other emission that roughly outlines the SNR shell. Figure 1a in \citet{duncan1996} shows the radio emission at 2.4GHz of the Vela region. Vela-X exhibits extreme radio emission and our shock sits on the outskirts (center shock position in galactic coordinates: $l$=262.527, $b$=-4.069). It is worth noticing the radio emission in the southwestern region is lacking in comparison to the northern region. This trend is consistent throughout radio observations. Observing $^{12}$CO emission at 115GHz revealed the same behavior of the Vela region \citep{mori2001}. The lack of emission in this region indicates a less dense ISM south of the PWN. This is also consistent with observations of the pulsar position and proper motion. The pulsar is known to be in the northern edge of the radio emission. The offset is likely caused by the expansion of the SNR into the ISM and how this interacts with the PWN. It is possible a non-uniform density in the ambient interstellar medium (ISM) is the cause of the asymmetric appearance \citep{hess2012} that causes an early return of the reverse shock of the SNR from the direction where the shock encounters a denser medium, in this case, the northern edge \citep{hess2012}. The atomic hydrogen density of 1-2 particles per cm$^3$ for the northern edge of the SNR is indeed greater than the estimated 0.1 particles per cm$^3$ in the southern ISM, supporting this observed appearance of the region (Dubner et al. 1998, Ferreira & de Jager 2008, Abramoswki et al 2012). 

\begin{figure}[!t]
\centering
\includegraphics[width=.75\linewidth]{24GHz_shock_ctr.png}
\caption{Zoom in of \citet{duncan1996} Figure 1a with contours of radio (green) and contours of X-ray shock (red).}\label{fig:radio}
\end{figure}

\citet{dubner1998} mapped 21cm HI clouds in the Vela region reporting negative radial velocities (-21 km s$^{-1}$ to -9 km s$^{-1}$). Later \citet{bach2000} connected the high $N_{H}$ column densities in the southern region with the HI clouds, and concluding that the HI clouds must be moving towards us and are likely being accelerated by the SNR shock wave. Dubner interpreted the HI presence as a bubble that the Vela SNR is expanding into with a higher interaction in the north and east directions. \citet{bach2000} has speculated that the interaction is weaker with HI in the south and west directions, allowing the shock wave to keep expanding inside the bubble. \citet{bach2000} also suggests that the high $N_{H}$ infers that cold interstellar gas lies behind the SNR in the south region and that it is likely for the HI clouds to be in front of the remnant in the west which may explain the apparent cavity that exists west of the XMM-Newton X-ray source.

Furthermore, a small HI cloud has been identified in \citet{dubner1998} that delineates the H$\alpha$ optical filament associated with the observed X-ray shock. The morphology of the filament correlates well with the location and size of the HI cloud in this region strongly suggesting that the shock is interacting with the cloud. Optical emission is usually indicative of bright X-ray boundary regions which is indeed what is observed on the ROSAT map. This may suggest a density enhancement in the western region and is also evidence of the forward shock of the Vela SNR.{\color{red} This poses some interesting questions as the shock is located on an inner boundary much closer to the pulsar than the distinguished 8$\degree$ diametter SNR shell. }

\subsection{$\gamma$-rays}
PWNe contribute significantly to the Galactic VHE $\gamma$-ray emission \citep{hess2012} and as previously noted, J0826-4500 was first discovered at E$>$50GeV. Recent observations of Vela-X in E$>$100GeV was reported by the H.E.S.S. collaboration, \citet{hess2012}, that challenges the idea that morphologies of X-ray and $\gamma$-ray emission should correspond to one another. The Vela region has since proven it is much more chaotic in structure as the radio extent of the PWN appears more consistent with the VHE $\gamma$-ray emission. The Fermi data of Vela-X over 4 years of observations \citep{grondin2013} shows morphological similarities with Wilkinson Microwave Anisotropy Probe (WMAP) radio emission at 61 GHz which provides direct evidence of low energy electron presence in the PWN. The PWN is large with significant emission seen up to 1$\degree$ from the pulsar in the $\gamma$-rays.

The extension of the X-ray source was tested using Fermi-LAT  using extended templates and disks of radius of 0.1, 0.2, 0.3, and 0.4 degrees around the source position. The Fermi-LAT extension test resulted in insignificant statistics. The LAT can resolve 6’ in size at E$>$50GeV, however, the X-ray source is very faint, producing a test statistic of 26 and estimated photon count between 4 and 5 so the results of the extension test are not so surprising. The test may be inconclusive whether the original $\gamma$-ray detection came from a portion or all of the shock but Fermi’s inability to resolve the shock structure is not so discouraging. Future efforts will include a deeper analysis in VHE.

Several scenarios have been suggested to explain the spatial, morphological, and spectral variations that exist throughout the region and will be discussed at length in section 4.  


\section{Discussion}
\subsection{Possible Origins}
As described in section 3, the shock is clearly sitting just on the western edge of the radio PWN where thermalization occurs at the wind termination shock \citep{steve2017}. Ions present in the pulsar winds are interacting with the magnetic field and the highly relativistic leptons causing the thermalization. A pressure balance lies between the pulsar wind outflow and the local ambient SNR plasma that fixes the location of the TS \citep{steve2017}. This is a probable explanation of the location of the X-ray source. Vela-X is considered a peculiar PWN as the pulsar powers several layers of wind nebulae throughout the SNR including the: compact X-ray nebula seen as two toroidal arcs that are small in structure and distance (subarcminute scale), the 4' helical jet, extended hard X-ray emission that is apparent north of the pulsar, a 45' soft X-ray \textit{cocoon} with TeV emission also detected in the same region, and finally, the Vela-X \textit{halo} that encompasses all of these layers in a 2$\degree$x3$\degree$ non-thermal region offset by approximately 40' from the pulsar that also exhibits GeV energies detected by Fermi \citep{steve2017}. 

The active and perplexed region likely has more than one particle population responsible for the variations observed. Here we discuss the possibilities for the particle populations at work.
One interpretation of the variations between energies throughout the region involves two lepton populations responsible for the different spectra of the cocoon and halo. One of these would be a younger population that produces the observed X-ray and VHE cocoon and the second population would be considerably older, perhaps as earlier injected particles from the pulsar, and resulting in the radio and HE halo. Both of these populations can emit at the observed energies in similar magnetic fields of 3-5$\mu$G \citep{steve2017}. However, recent observations from H.E.S.S. challenge this scenario, having revealed that there is TeV emission within the cocoon and into the halo. The TeV emission was found to be spatially coincident with \textit{WMAP} 61 GHz radio maps of the region, however, the northern and southern \textit{wings} of the radio emission have marginally different spectra as the northern wing is seen to be weaker above 1GeV indicating a softer spectrum than the southern wing \citep{grondin2013}. 

The new Fermi-LAT observations from \citet{grondin2013} shows a striking relationship between the GeV and radio emission, providing direct evidence of low energy electrons present in the extended halo. There is significant emission seen up to 1$\degree$ from the pulsar. Additionally, the large size of the PWN could be explained by an electron population that is not coming from the pulsar at all but is instead accelerated in the extended halo and stochastically accelerated due to the turbulent magnetic fields in the outer PWN or in the ambient SNR plasma. However, this scenario does not support the development of shocks in the halo so this is an unlikely explanation for the X-ray source. 

A more likely scenario is that the high energy electrons are diffusively escaping (originally invoked by Hinton et al 2011). It is likely that the reverse shock (RS) of the SNR has already passed over the pulsar which has caused a diffusion of particles out of the nebula and creating a mildly supersonic flow \citep{steve2017, grondin2013, bs2017}. The diffusive escape would be rapid with an escape time of $T\approx90(\frac{R}{10pc})^{2}(\frac{E}{100TeV}^{-1}) yrs$ \citep{grondin2013} where R is the radius of the PWN and E is the electron energy. \citet{grondin2013} reports this escape time is 1000 times faster than Bohm diffusion.  This scenario challenges the common assumption of toroidal magnetic fields with strong confinement but can recover if the RS passage causes mixing and turbulence causing a disruption in the magnetic field structure and this can allow the rapid diffusion of particles.

The diffusion theory is a common explanation as it can also explain the location of our source. It could be indicative to the pulsar's past activity - the HE electrons that were injected by the pulsar when it was younger. This was used in Hinton et al 2011 to interpret past Fermi data of the outskirts of Vela-X and was also included in \citet{bs2017} that can account for particle escape, transport, and magnetic field structure that again leads back to the disturbances resulting from the RS passage. However, the use of the rapid diffusion scenario in Hinton et al 2011 cannot describe the TeV emission seen at large distances away from the pulsar because the electrons would escape too fast. \citep{grondin2013} suggests that the injection of two electron populations with decreasing diffusion time could resolve this, enabling 10TeV photons to be visible up to 10pc away from the pulsar in a 5$\mu$G magnetic field. This revision slows the diffusion rate to only 20 times the Bohm diffusion rate. 

The rapid diffusion scenario should produce spectral differences in the inner and outer regions of the PWN due to radiative cooling of the electrons as they propagate and this contradicts H.E.S.S. observations as the spectral variation in the TeV range is absent \citep{grondin2013}. To account for this, perhaps the diffusive particle escape is energy dependent and stochastic re-acceleration may be occuring in the radio halo. This may explain the H.E.S.S. observations in TeV and its connection to radio and $\gamma$-ray emission. The diffusive particle escape theory further suggests that the $\gamma$-ray emission should soften as distance from pulsar grows. The X-ray shock, however, has a hard $\gamma$-ray photon index. 

If rapid diffusion is in fact occurring due to the RS passage, this mixing could cause a shock front as the particles escape into the surrounding SNR plasma. This may explain the X-ray shock that is seen just on the edge of the PWN. 

Another possibility includes relativistic ions colliding inelastically with thermal gas and producing charged neutral pions. The $\pi^{0}$ mesons decay to photons and generates energy at 150MeV and above \citep{steve2017}. This could explain the thermal origin of the X-ray shock,however, it is not a major contributer to the higher energy spectra of PWN - but in our case, the X-ray shock is small relative to the rest of the region so this could be the result of small ion collisions. 

A combination of mechanisms is also possible. The particles may be diffusively escaping as previously mentioned in addition to the movement and expansion of the PWN into the SNR. As the surrounding ejecta interacts with the wind, it becomes heated and forms a shock. The shock gains considerable heat as it moves into the HI region and interacts with the small cloud as discussed in \citet{dubner1998}. 

\section{Conclusion}

\section{Acknowledgements}
We would like to thank Alberto Dominguez for testing the $\gamma$-ray extension of J0826-4500. We would also like to thank Daniel Castro at Harvard University for his expertise and guidance on gathering data for the characterization of the source. 

